Shapes and Norms of Random Pairs

The shape function of a pair of finite-valued random variables was introduced in arXiv:2606.23849, where it was used to derive a spectral bound on the entanglement of the pair, a quantity measuring the extent to which their mutual information can be extracted. In this article, we further develop the theory of shape functions for pairs of random variables. We prove that, when $(X,Y)$ is uniformly supported on the edges of a biregular bipartite graph, the value of the shape function $\mathcal{S}(X,Y)(\alpha,\beta)$ equals the logarithm of the operator norm of the graph's incidence matrix with respect to Lebesgue exponents determined by $(\alpha,\beta)$.This identification, in particular, enables the numerical approximation of the shape function and, by duality, of the extension profile, also known as the tension region, of the pair. We also establish a collection of relations and inequalities satisfied by shape functions, including convexity and monotonicity properties, composition inequalities, and relations describing their behavior under conditioning and the adjoining of variables.

==> defs.tex <==
\makeatletter


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Editing

%skip arguments
\newcommand{\skipthis}[2][]{\relax}
\let\comment=\skipthis

% skip the next par
\long\def\skippar#1\par{\relax\par}

\usepackage{xcolor}
\def\exclam#1{\ifmmode\relax\else\marginpar{\textcolor{#1}{\fbox{!!!}}}\fi}
% \def\exclam#1{\relax}
% colored text
\long\def\red#1{{\textcolor{red}{\exclam{red}#1}}}
\long\def\green#1{\textcolor{green}{#1}}
\long\def\blue#1{{\textcolor{blue}{\exclam{blue}#1}}}
\long\def\cyan#1{\textcolor{cyan}{\exclam{cyan}#1}}
\long\def\brown#1{\textcolor{brown}{#1}}
\long\def\green#1{\textcolor{green}{#1}}
\long\def\lime#1{\textcolor{lime}{#1}}
\long\def\magenta#1{\textcolor{magenta}{#1}}
\long\def\olive#1{\textcolor{olive}{#1}}
\long\def\pink#1{\textcolor{pink}{#1}}
\long\def\purple#1{\textcolor{purple}{#1}}
\long\def\teal#1{\textcolor{teal}{#1}}
\long\def\violet#1{\textcolor{violet}{#1}}
\long\def\yellow#1{\textcolor{yellow}{#1}}
\long\def\orange#1{\textcolor{orange}{#1}}
\long\def\gray#1{\textcolor{gray}{\exclam{gray} #1}}\let\grey=\gray


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Letters

%%% I like \varphi and \varepsilon better then the standard
\let\tmp=\phi \let\phi=\varphi \let\varphi=\tmp
\let\tmp=\epsilon \let\epsilon=\varepsilon \let\varepsilon=\tmp

%%% Define all modified face or accented letters, eg \xbf for boldface x
%%% \Rbb for \mathbb{R}, \xtilde, \yhat, \zsf, etc.

\newcommand{\bmmax}{2}
\usepackage{bm}
\def\imathbf{{\bm\imath}}
\def\jmathbf{{\bm\jmath}}

%% Math letters, fonts and deco
%% Define \<letter><font> 

\def\mathun#1{\underline{#1}}
\def\mathov#1{\overline{#1}}
\def\mathbar#1{\bar{#1}}
\def\mathhat#1{\hat{#1}}
\def\mathwh#1{\widehat{#1}}
\def\mathtilde#1{\tilde{#1}}
\usepackage{accents}
\def\mathdtilde#1{\accentset{\approx}{#1}}


\def\mkmathletter#1#2{%
    \expandafter\gdef\csname#1#2\endcsname%
           {\ensuremath{\csname math#2\endcsname{#1}}}%
}

\edef\letters{a,b,c,d,e,f,g,h,i,j,k,l,m,n,o,p,q,r,s,t,u,v,w,x,y,z}
\edef\Letters{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}
\edef\Lletters{\letters,\Letters}

\def\mkmathletters#1#2{%
        \@for\ltr:={#2}\do{\expandafter\mkmathletter\ltr{#1}}%
}

% \mkmathletters{frak}{\Lletters} %\Afrak, \bfrak
% \mkmathletters{un}{\Lletters}   % underlined
% \mkmathletters{ov}{\Lletters}   % overlined
% \mkmathletters{wh}{\Lletters}   % with wide hat
% \mkmathletters{hat}{\Lletters}  % hat
% \mkmathletters{tilde}{\Lletters}% with tilde


\edef\greek{alpha,beta,gamma,delta,epsilon,zeta,eta,theta,jota,kappa,lambda,%
  mu,nu,xi,pi,omikron,rho,sigma,tau,upsilon,varphi,phi,chi,psi,omega}
\edef\Greek{Alpha,Beta,Gamma,Delta,Epsilon,Zeta,Eta,Theta,Jota,Kappa,%
  Lambda,Mu,Nu,Xi,Pi,Omikron,Rho,Sigma,Tau,Upsilon,Varphi,Phi,Chi,%
  Psi,Omega}
\edef\Ggreek{\greek,\Greek}

\def\mkboldgreek#1;{\expandafter\def\csname#1bf\endcsname{%
    \expandafter\bm\csname#1\endcsname}}

\def\mkbolds#1{%
  \@for\ltr:={#1}\do{\expandafter\mkboldgreek\ltr;}%
}

\def\mksfgreek#1;{\expandafter\def\csname#1sf\endcsname{%
    \expandafter\mathsf{\csname#1\endcsname}}}

\def\mksf#1{%
  \@for\ltr:={#1}\do{\expandafter\mksfgreek\ltr;}%
}

% \mkbolds{\Ggreek}
% \mksf{\Ggreek}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% Arrows
\newcommand{\into}[1][]{\stackrel{#1}{\hookrightarrow}}
\renewcommand{\to}[1][]{\stackrel{#1}{\rightarrow}}
\newcommand{\too}[1][]{\stackrel{#1}{\longrightarrow}}
\newcommand{\ot}[1][]{\stackrel{#1}{\leftarrow}}
\newcommand{\oot}[1][]{\stackrel{#1}{\longleftarrow}}
\newcommand{\oto}[1][]{\stackrel{#1}{\leftrightarrow}}
\newcommand{\ootoo}[1][]{\stackrel{#1}{\longleftrightarrow}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Binary Ops

\def\indep{\,\makebox[0cm][l]{$\bot$}\,\bot\,}

% Brackets
\def\<{\left\langle}
\def\>{\right\rangle}
\def\cl#1{\left\lceil#1\right\rceil}
\def\fl#1{\left\lfloor#1\right\rfloor}
\def\vect#1{\left(\!\!\!\begin{array}{c}#1\end{array}\!\!\!\right)}
\def\sep{|\mkern-2mu|}
\newcommand{\iso}[1][]{\stackrel{#1}{\cong}}
% set
\def\st{\;{\bm :}\;}
\def\set#1{\left\{#1\right\}}

\def\dx{\mathrm{d}x}
\def\dy{\mathrm{d}y}
\def\dz{\mathrm{d}z}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Math Operators
\let\dmo=\DeclareMathOperator

\makeatother

